The Production and Consumption of Social Media

We model social media as collections of users producing and consuming content. Users value consuming content, but doing so uses up their scarce attention, and hence they prefer content produced by more able users. Users also value receiving attention, creating the incentive to attract an audience by producing valuable content, but also through attention bartering -- users agree to become each others' audience. Attention bartering can profoundly affect the patterns of production and consumption on social media, explains key features of social media behavior and platform decision-making, and yields sharp predictions that are consistent with data we collect from EconTwitter.

==> Makefile <==
project_name = twitter

ts := $(shell /bin/date "+%Y-%m-%d---%H-%M-%S")

plots      = 
parameters = 
tables     = 


package_list.txt:
	 find ../analysis/ -name '*R' -print0 | xargs -0 grep -h 'library*' | sed 's/library//g' | sed 's/#//g' | sed 's/ //g' | sort | uniq| sed 's/(//g' | sed 's/)//g' > package_list.txt

install_packages: package_list.txt
	cat package_list.txt | xargs -I {} Rscript -e 'install.packages("{}")'

## This project uses several datasets#############

# -- input file contains variables and libraries
input            = ../analysis/input.R 

# raw data
repec            = ../data/raw/repec_economists.rds
seeds            = ../data/raw/data_seeds.rds
data             = ../data/raw/data.csv
relation         = ../data/raw/relation.csv

# -- clean data
repec_clean      = ../data/temp/repec_economists.csv
seeds_clean      = ../data/temp/data_seeds.csv
data_clean       = ../data/temp/data.csv

# -- reduced data
users_economists_active    = ../data/temp/users_economists_active.csv
users_all_active           = ../data/temp/users_all_active.csv
relation_economists_active = ../data/temp/relation_economists_active.csv
relation_all_active        = ../data/temp/relation_all_active.csv

# -- reciprocation stats
reciprocation     = ../data/temp/reciprocation.csv
reciprocation_all = ../data/temp/reciprocation_all.csv


#############################
## 1. Homogeneous preferences
#############################

## --- 1.1 No follower information

# compute followers an utilities
../computed_objects/no_info_uniform_followers.csv ../computed_objects/no_info_uniform_utilities.csv: ../analysis/no_info_uniform.py $(input)
	cd ../analysis && ./no_info_uniform.py

# plot followers
plots += ./plots/no_info_uniform_followers.pdf
./plots/no_info_uniform_followers.pdf: ../analysis/no_info_uniform_followers.R ../computed_objects/no_info_uniform_followers.csv $(input)
	cd ../analysis && ./no_info_uniform_followers.R

# plot utilities
plots += ./plots/no_info_uniform_utilities.pdf
./plots/no_info_uniform_utilities.pdf: ../analysis/no_info_uniform_utilities.R ../computed_objects/no_info_uniform_utilities.csv $(input)
	cd ../analysis && ./no_info_uniform_utilities.R

## --- 1.2 Follower information

# compute followers, utilities, and ratio
../computed_objects/info_uniform_followers.csv ../computed_objects/info_uniform_utilities.csv ../computed_objects/info_uniform_ratio.csv: ../analysis/info_uniform.py $(input)
	cd ../analysis && ./info_uniform.py

# plot followers
plots += ./plots/info_uniform_followers.pdf
./plots/info_uniform_followers.pdf: ../analysis/info_uniform_followers.R ../computed_objects/info_uniform_followers.csv $(input)
	cd ../analysis && ./info_uniform_followers.R

# plot utilities
plots += ./plots/info_uniform_utilities.pdf
./plots/info_uniform_utilities.pdf: ../analysis/info_uniform_utilities.R ../computed_objects/info_uniform_utilities.csv $(input)
	cd ../analysis && ./info_uniform_utilities.R

# plot ratio
plots += ./plots/info_uniform_ratio.pdf
./plots/info_uniform_ratio.pdf: ../analysis/info_uniform_ratio.R ../computed_objects/info_uniform_ratio.csv $(input)
	cd ../analysis && ./info_uniform_ratio.R


#############################
## 2. Heterogeneous preferences
#############################

## --- 2.1 Het no follower information

# compute followers and utilities
../computed_objects/het_no_info_uniform_followers.csv ../computed_objects/het_no_info_uniform_utilities.csv: ../analysis/het_no_info_uniform.py $(input)
	cd ../analysis && ./het_no_info_uniform.py

# plot followers
plots += ./plots/het_no_info_uniform_followers.pdf
./plots/het_no_info_uniform_followers.pdf: ../analysis/het_no_info_uniform_followers.R ../computed_objects/het_no_info_uniform_followers.csv $(input)
	cd ../analysis && ./het_no_info_uniform_followers.R

# plot utilities
plots += ./plots/het_no_info_uniform_utilities.pdf
./plots/het_no_info_uniform_utilities.pdf: ../analysis/het_no_info_uniform_utilities.R ../computed_objects/het_no_info_uniform_utilities.csv $(input)
	cd ../analysis && ./het_no_info_uniform_utilities.R

## --- 2.2 Het follower information

# compute followers, utilities, reciprocation range, and ratio
../computed_objects/het_info_uniform_followers.csv ../computed_objects/het_info_uniform_utilities.csv ../computed_objects/het_info_uniform_ratio.csv: ../analysis/het_info_uniform.py $(input)
	cd ../analysis && ./het_info_uniform.py

# plot followers
plots += ./plots/het_info_uniform_followers.pdf
./plots/het_info_uniform_followers.pdf: ../analysis/het_info_uniform_followers.R ../computed_objects/het_info_uniform_followers.csv $(input)
	cd ../analysis && ./het_info_uniform_followers.R

# plot utilities
plots += ./plots/het_info_uniform_utilities.pdf
./plots/het_info_uniform_utilities.pdf: ../analysis/het_info_uniform_utilities.R ../computed_objects/het_info_uniform_utilities.csv $(input)
	cd ../analysis && ./het_info_uniform_utilities.R

# plot reciprocation
#plots += ./plots/het_info_uniform_reciprocation.pdf
#./plots/het_info_uniform_reciprocation.pdf: ../analysis/het_info_uniform_reciprocation.R ../computed_objects/het_info_uniform_reciprocation.csv $(input)
#	cd ../analysis && ./het_info_uniform_reciprocation.R

# plot ratio
plots += ./plots/het_info_uniform_ratio.pdf
./plots/het_info_uniform_ratio.pdf: ../analysis/het_info_uniform_ratio.R ../computed_objects/het_info_uniform_ratio.csv $(input)
	cd ../analysis && ./het_info_uniform_ratio.R


#############################
## 3. Data
#############################

## --- 3.1 Clean data, generate new data, and compute params

# 3.1.1 keep only relevant attributes and rename variables
$(repec_clean) $(seeds_clean) $(data_clean): ../analysis/econtwitter_preprocessing_1.R $(input) $(repec) $(seeds) $(data)
	cd ../analysis && ./econtwitter_preprocessing_1.R

# 3.1.2 make datasets containing only active and non superstar accounts
$(users_economists_active) $(users_all_active) $(relation_economists_active) $(relation_all_active): ../analysis/econtwitter_preprocessing_2.R $(input) $(repec_clean) $(seeds_clean) $(data_clean) $(relation)
	cd ../analysis && ./econtwitter_preprocessing_2.R

# 3.1.3 compute reciprocation statistics for econtwitter users WITHIN #ECONOTWITTER --- only econ-to-econ relationships
#$(reciprocation): ../analysis/econtwitter_preprocessing_3.py $(users_economists_active) $(relation_economists_active)
#	cd ../analysis && ./econtwitter_preprocessing_3.py

# 3.1.4 compute reciprocation statistics for econtwitter users WITH ALL OTHER USERS --- econ-to-everyone relationships
$(reciprocation_all): ../analysis/econtwitter_preprocessing_4.py $(users_economists_active) $(users_all_active) $(relation_all_active)
	cd ../analysis && ./econtwitter_preprocessing_4.py


## --- 3.2 Plots

# 3.2.1 plot kernel density distribution estimates on ECONTWITTER sample
plots += ./plots/econtwitter_stats_distr.pdf
./plots/econtwitter_stats_distr.pdf: ../analysis/econtwitter_stats_distr.R $(input) $(users_economists_active)
	cd ../analysis && ./econtwitter_stats_distr.R

# 3.2.3 plot equilibrium predictions of statistics of users as a function of user ability
plots += ./plots/theory_stats_ability.pdf 
./plots/theory_stats_ability.pdf: ../analysis/theory_stats_ability.R $(input) ../computed_objects/info_uniform_ratio.csv
	cd ../analysis && ./theory_stats_ability.R

# 3.2.4 plot statistics of econtwitter users as a function of user ability
plots += ./plots/econtwitter_stats_ability.pdf 
./plots/econtwitter_stats_ability.pdf: ../analysis/econtwitter_stats_ability.R $(input) $(users_economists_active)
	cd ../analysis && ./econtwitter_stats_ability.R

# 3.2.5 plot reciprocation statistics as a function of user ability
plots += ./plots/econtwitter_stats_reciprocation.pdf 
plots += ./plots/econtwitter_stats_reciprocation_range.pdf 
./plots/econtwitter_stats_reciprocation.pdf ./plots/econtwitter_stats_reciprocation_range.pdf : ../analysis/econtwitter_stats_reciprocation.R $(input) $(reciprocation_all)
	cd ../analysis && ./econtwitter_stats_reciprocation.R

# 3.2.6 plot MODEL predictions of reciprocation statistics as a function of user ability
plots += ./plots/model_stats_reciprocation_range.pdf 
./plots/model_stats_reciprocation.pdf ./plots/model_stats_reciprocation_range.pdf : ../analysis/model_stats_reciprocation.R $(input) $(users_economists_active)
	cd ../analysis && ./model_stats_reciprocation.R

# 3.2.B plot a BIG BADA PLOT
plots += ./plots/bigbadaplot.pdf 
plots += ./plots/bigbadaplot_unscaled.pdf 
./plots/bigbadaplot.pdf ./plots/bigbadaplot_unscaled.pdf: ../analysis/bigbadaplot.R $(input) ../computed_objects/info_uniform_ratio.csv $(users_economists_active) $(reciprocation_all)
	cd ../analysis && ./bigbadaplot.R

#############################
## 4. Parameters
#############################

## --- 4.1 General parameters

# compute parameters
parameters += ./parameters.tex
./parameters.tex: ../analysis/parameters.R $(input) $(seeds_clean) $(users_economists_active) $(users_all_active)
	cd ../analysis && ./parameters.R


#############################
## 5. Appendix
#############################

## --- 5.1 Plots

# 5.1.2 plot statistics of all users as a function of user ability on ALL sample
#plots += ./plots/alltwitter_stats_ability.pdf 
#./plots/alltwitter_stats_ability.pdf: ../analysis/alltwitter_stats_ability.R $(input) $(users_all_active)
#	cd ../analysis && ./alltwitter_stats_ability.R

# 5.1.2 plot kernel density distribution estimates on ALL sample 
plots += ./plots/alltwitter_stats_distr.pdf
./plots/alltwitter_stats_distr.pdf: ../analysis/alltwitter_stats_distr.R $(input) $(users_all_active)
	cd ../analysis && ./alltwitter_stats_distr.R

## --- 5.2 Tables

# 5.2.1 ability is not correlated with when user joined
tables += ./tables/age_ability.tex
./tables/age_ability.tex: ../analysis/age_ability.R $(input) $(users_economists_active) $(reciprocation_all)
	cd ../analysis && ./age_ability.R


#############################
## 6. Make commands
#############################

## --- 6.1.1 Makes or updates manuscript using latex & bibtext
$(project_name).pdf: $(project_name).bib $(project_name).tex $(plots) $(parameters) $(tables)
	pdflatex -interaction=batchmode $(project_name)
	bibtex $(project_name)
	pdflatex -interaction=batchmode $(project_name)
	pdflatex -interaction=batchmode $(project_name) 


## --- 6.1.2 Makes paper from scratch
clean:	
	rm -f plots/*
	rm -f tables/*
	rm -f parameters.tex
	rm -f $(project_name).pdf
	rm -f $(project_name).aux
	rm -f $(project_name).bbl
	rm -f $(project_name).blg
	rm -f $(project_name).log
	rm -f $(project_name).out
	rm -f ../computed_objects/*.rds
	rm -f ../computed_objects/*.csv
	rm -f ../data/temp/*
	make $(project_name).pdf

## --- 6.2.1 Uploads to JJHs dropbox
toread: $(project_name).pdf
	scp $(project_name).pdf bandit-local.local:~/Dropbox/toread/$(project_name)_$(ts).pdf 

## --- 6.2.2 Uploads to JJHs remote
toread_bandit: $(project_name).pdf
	scp $(project_name).pdf bandit:/home/ubuntu/Dropbox/toread/$(project_name)_$(ts).pdf 

## --- 6.3.1 Makes local backup
../backups/$(project_name)_$(ts).tar.gz:
	tar --exclude='../backups' --exclude='../.git' -zcvf ../backups/$(project_name)_$(ts).tar.gz ../

backup: ../backups/$(project_name)_$(ts).tar.gz
	echo "Making backup"

## --- 6.3.2 Makes remote backup
backup_s3: ../backups/$(project_name)_$(ts).tar.gz
	aws s3 cp ../backups/$(project_name)_$(ts).tar.gz s3://john_horton_backups/

backup_glacier: ../backups/$(project_name)_$(ts).tar.gz
	aws glacier upload-archive --account-id - --vault-name backups --archive-description $(project_name)_$(ts).tar.gz --body  ../backups/$(project_name)_$(ts).tar.gz >> ../backups/glacier_history.txt

snapshot:
	@echo Timestamp is $(ts)
	cp $(project_name).pdf ../snapshots/$(project_name)_$(ts).pdf

## --- 6.4 Uploads to JJhs website
website: $(project_name).pdf
	printf 'cd papers\nput $<\n' \ | sftp -oPort=2222 -oCiphers=aes256-ctr johnjhorton@104.198.96.220
